Reward Shaping for Building Trustworthy Robots in Sequential Human-Robot Interaction

Trust-aware human-robot interaction (HRI) has received increasing research attention, as trust has been shown to be a crucial factor for effective HRI. Research in trust-aware HRI discovered a dilemma -- maximizing task rewards often leads to decreased human trust, while maximizing human trust would compromise task performance. In this work, we address this dilemma by formulating the HRI process as a two-player Markov game and utilizing the reward-shaping technique to improve human trust while limiting performance loss. Specifically, we show that when the shaping reward is potential-based, the performance loss can be bounded by the potential functions evaluated at the final states of the Markov game. We apply the proposed framework to the experience-based trust model, resulting in a linear program that can be efficiently solved and deployed in real-world applications. We evaluate the proposed framework in a simulation scenario where a human-robot team performs a search-and-rescue mission. The results demonstrate that the proposed framework successfully modifies the robot's optimal policy, enabling it to increase human trust at a minimal task performance cost.

==> backup/multi-objective_Optimization_Version.tex <==
\input{header}


\begin{document}



\maketitle
\thispagestyle{empty}
\pagestyle{empty}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}

This electronic document is a ÒliveÓ template. The various components of your paper [title, text, heads, etc.] are already defined on the style sheet, as illustrated by the portions given in this document.
\cite{Azevedo_context}
\end{abstract}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\yao{hyperref does not work}
Trust has been identified as a crucial factor for successful human-robot interaction (HRI), which is essential for safe and reliable functioning of robots, social acceptance, and effective collaboration~\cite{Sheridan:2016kn, Azevedo_context, Yang:2017:EEU:2909824.3020230, du2020not}.

To enable effective trust-aware human-robot interaction (HRI), two research directions have been proposed. The first direction, known as trust calibration, assumes that there exists an optimal trust value, referred to as the trust calibration point, that a human operator should have in a robot~\cite{lee2004trust}. The failure to reach this calibration point would result in decreased task performance due to either "distrust" if the human trust is below the calibration point, leading to underutilization of the robot's capabilities, or "overtrust" if human trust is above the calibration point, causing the human to reduce their situational awareness and over-rely on the robot. Trust calibration aims to identify the calibration point and guide human trust towards it.

The second direction, trust-aware planning, has been proposed in recent years, with the aim of enabling the robot to explicitly consider the human's trust in its decision-making process \cite{chen2020trust}. In their work, Chen et al. modeled the human-robot interaction process as a POMDP, where human trust is considered part of the environment state. They further integrated human trust dynamics into the state transition function, allowing the robot to optimize its objective in the interaction process by leveraging human trust without relying on predefined calibration points. However, the authors found that maximizing task rewards often leads to decreased human trust, while maximizing human trust would compromise task performance.

Guo further investigated the behavior of robots in trust-aware planning when facing different human conditions, showing that trust-aware planning could even lead to the robot deliberately lying to its human partner~\cite{guo2021reverse}. To mitigate this, they proposed adding an additional "trust-seeking" term to the reward function to encourage the robot to increase human trust and avoid lying. However, this additional reward term takes the form of a simple indicator function of the robot's performance, and it remains unclear what types of trust reward terms would lead to better task performance and increased human trust, and how to compute such terms.

In this work, we address the trust-aware human-robot interaction problem by formulating it as a bi-objective optimization. To balance the two objectives, we convert the problem into an epsilon-constraint problem and propose a novel reward-shaping method to solve it. Specifically, we apply the proposed framework on the experience-based trust model, resulting in an elegant linear program that can be efficiently solved and deployed in real-world applications. We evaluate the proposed framework in a simulation scenario where a human-robot team performs a search-and-rescue mission. The results demonstrate that the proposed framework successfully modifies the robot's optimal policy, enabling it to increase human trust with minimal task performance cost.

The contributions of this work include:
\begin{itemize}
    \item Proposing a computational framework for designing trustworthy interaction policies for trust-aware robots.
    \item Developing a novel reward-shaping method for designing the trust-seeking term.
\end{itemize}

In the remainder of this paper, we review relevant literature in Section 2. In Section 3, we formulate the trust-aware human-robot interaction problem as a two-player Markov game and discuss the problem in a multi-objective optimization setting. In Section 4, we present the reward shaping method for designing the trust-seeking term. In Section 5, we present the simulation scenario used to evaluate the proposed framework. Finally, in Section 6, we discuss the results and summarize the work.

% Recent advances in autonomous systems, such as autonomous vehicles and collaborative robots, have the potential to improve every sector of our economy and improve how people live and work. However, realizing the full potential of these technologies is only possible if people establish appropriate trust in them \cite{Sheridan:2016kn, Azevedo_context, Yang:2017:EEU:2909824.3020230, du2020not}.

% To facilitate effective trust-aware HRI, two lines of research have been proposed. The first line is trust calibration, where researchers assume that there is an optimal trust value, called the trust calibration point, that a human operator should have in a robot. For instance, uncalibrated trust would lead to decreased task performance: \textit{distrust} occurs if human trust is below the calibration point, resulting in the failure to take full advantage of the robot's capabilities; \textit{overtrust} occurs when human trust is above the calibration point, causing the human to decrease their situational awareness and overly rely on the robot. As a result, trust calibration focuses on identifying the calibration point and guiding human trust to it.


% The second line is trust-aware planning, proposed in recent years, aiming to enable the robot to explicitly consider the human's trust in its decision-making process \cite{chen2020trust}. In XXX, the authors modeled the human-robot interaction process as a POMDP where the human trust is part of the environment state and integrated human trust dynamics in the state transition function. Such a trust-aware planning mechanism allows the robot to optimize its objective in the interaction process by taking advantage of human trust, while do not need a predefine calibration point. However, the authors found that the maximize task reward often leads to decreased human trust, while maximizing human trust would compromise task performance. Guo further examined robot's behavior in trust-aware planning when facing different human, showing that trust-aware planning can even cause the robot to deliberatively lie to its human partner. They proposed to add an additional trust-seeking term in the reward function to encourage the robot to increase human trust and thus not lie. However, this additional reward term takes the form of a simple indicator function of the robot's performance, it remains unknown what types of trust reward terms would lead to better task performance and increased human trust and how to compute such terms.

% To fill this gap, in this work, we consider the trust-aware human-robot interaction problem as a bi-objective optimization. We convert the problem of balancing the two objectives to an epsilon-constraint problem and proposed a novel reward-shaping method to solve the problem. In particular, applying the proposed framework to the experience-based trust model results in an elegant linear program, which can be solved efficiently and thus be readily deployed in real-world applications. We analyze the proposed framework in a simulation, where a human-robot team works on a search-and-rescue mission. Results show the proposed framework successfully modified the robot's optimal policy, allowing the robot to increase human trust at a minimal cost of task performance.

% The contributions of this work include:
% propose a computational framework for designing trustworthy interaction policy for trust-aware robots; develop a novel reward-shaping method for designing the trust-seeking term.

% The remaining contents are organized as follows: we first review relevant literature in section 2; in section 3, we formulate the trust-aware human-robot interaction problem as a two-player Markov game and discuss the problem in a multi-objective optimization setting; in section 4, we present the reward shaping method for designing the trust-seeking term; in section 5, we present a simulation to test the proposed framework; finally, in section 6, we discuss the results and summarize the work. 

% =================================

%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%








% The success of trust-aware HRI depends on two components: the trust dynamics model and the trust-behavior model. A trust dynamics model specifies how a human's trust changes in response to moment-to-moment interaction with a robot \cite{Guo2020_IJSR}. A trust-behavior model describes the human's behavior as a function of trust. Note that trust and behavior are distinct constructs: trust in autonomy is the ``attitude that an agent will help achieve an individual's goals in situations characterized by uncertainty and vulnerability \cite{See:2004vj}" while behavior is the human's compliance and reliance behavior, which is affected by his or her attitude.

% \textcolor{black}{Active research has been conducted to examine the trust dynamics model. Researchers have proposed computational models for inferring a human's trust in a robotic agent at any time based on the robot's performance, the human's behavioral information, and physiological information \cite{Guo2020_IJSR, xu2015optimo, Lu2020, hu2016real,Azevedo-Sa2020}. Little research, however, has investigated the trust-behavior model. Previous research largely assumed a disuse trust-behavior model~\cite{chen2020trust}, wherein a human will stop relying on a robot when his or her trust in the robot is low. However, psychological research has shown that people may display reverse-psychology behaviors~\cite{macdonald2011people}, which means a human will do exactly the opposite of what the robot suggests.}


% In this study, we simulate and compare how the disuse and the reverse psychology models affect trust-aware decision making and the human-robot team's performance. Results indicate that the robot will display certain ``manipulative'' behavior 
% % if the human's trust at low-trust states 
% if it assumes the human uses the reverse psychology model. Although this ``manipulative'' behavior may seem beneficial to the task performance in a short term, it could eventually undermine the human-robot interaction in the long run, e.g., leading to the disuse of the robot. To overcome such \textcolor{black}{``manipulative''} behaviors, we propose a trust-seeking reward function to prevent the robot from actively guiding the human to reduce his or her trust in order to take advantage of the reverse psychology behavior. We suggest augmenting a reward for gaining the human's trust in the short term, which will result in large benefits in the long run. 
% % We also find that under certain conditions, a Nash equilibrium occurs when both parties assume the disuse model. To the best of our knowledge, our study is the first attempt to study the trust-behavior models in computational settings, which paves the way for many future studies and applications.

% The rest of the paper is organized as follows: Section~\ref{sec:relatedWork} reviews related work in trust-driven human-robot interaction; Section~\ref{sec:model} formulates the trust-aware decision making problem in a POMDP framework and describes the trust-behavior model as well as the trust-seeking reward function;  Section~\ref{sec:case} introduces a reconnaissance mission as a study case to examine how different settings affect the interaction; Section~\ref{sec:result} reports the simulation results and our observations; Section~\ref{sec:discussion} summarizes our findings and discussed the limitations and future directions of this study. 

% \vfill

%===================================================
%===================================================
\section{Related Work}\label{sec:relatedWork}
% In this work, we aim to design rewards for trustworthy robots in HRI scenarios where the robot needs to balance its task performance and human trust. To achieve this, we formulate the HRI scenario as a two-player Markov game. Our framework builds on previous work on trust-aware HRI, which includes research on human trust in robots, trust-aware decision-making, as well as multi-objective optimization and reward shaping. In this section, we review relevant literature related to our proposed work.

In this work, we focus on reward design for trustworthy robots in sequential decision-making in HRI. The proposed work formulates the HRI scenario as a two-player Markov game, where the robot needs to balance its task performance and human trust. This framework is developed upon previous work on trust-aware HRI, including research on human trust in robots and trust-aware decision-making, as well as multi-objective optimization and reward shaping. We review relevant literature in this section.

Trust has been extensively studied in different areas and given different definitions. In the context of HRI, we will use the definition given by Lee and See: "trust is the attitude that an agent will help achieve an individual’s goals in a situation characterized by uncertainty and vulnerability".

\subsection{Computational Trust Model in HRI}
Previous literature attempted to understand the development and evolution of human trust in an HRI process. One area is to identify and quantify the factors that affect human trust. \cite{hancock2021evolving} classified such factors into three categories, namely human-related factors such as personality~\cite{Bhat_RAL_2022}, robot-related factors such as reliability~\cite{Lyons_HFJ_2021, gombolay_robotic_2018} and transparency~\cite{Wang:2016ui}, and task-related factors such as task emergency~\cite{Robinette:2016_HRI}. Another area aims to understand the temporal dynamics of trust when a person interacts with autonomy repeatedly~\cite{Yang2021_HFJ, DeVisser_IJSR, Guo2020_IJSR}. Empirical studies have investigated how trust strengthens or decays due to moment-to-moment interactions with autonomy~\cite{Lee:1992it, manzey2012human, Yang2021_HFJ, Yang:2017:EEU:2909824.3020230}. Based on these studies,~\cite{Guo2020_IJSR, Yang2021_chapter} summarized three major properties of trust dynamics: \textit{continuity}, \textit{negativity bias}, and \textit{stabilization}. 

\yao{this paragraph needs rewrite}
With these findings, several computational trust models have been developed~\cite{Xu2015optimo,  Guo2020_IJSR, wang2016impact}. Notably, Xu and Dudek~\cite{Xu2015optimo} proposed the online probabilistic trust inference model (OPTIMo) utilizing Bayesian networks to estimate human trust based on the autonomous agent's performance and human behavioral signals. Hu et al.~\cite{hu2016real} tested multiple binary trust classifiers based on human participants' electroencephalography (EEG) and galvanic skin response (GSR) signals and combined them into a voting classifier. Guo and Yang~\cite{Guo2020_IJSR} modeled trust as a Beta random variable parameterized by positive and negative interaction experience a human agent has with a robotic agent. Soh et al.~\cite{soh2020multi} proposed a Bayesian model which combines Gaussian processes and recurrent neural networks to predict trust over different tasks.

% To model trust dynamics and predict a human's trust in real time, prior work has proposed several trust estimators. Lee and Moray~\cite{Lee:1992it} proposed the auto-regressive moving average vector (ARMAV) model calculating trust as a function of task performance and the occurrence of automation failures. Xu and Dudek~\cite{xu2015optimo} built the online probabilistic trust inference model (OPTIMo) based on the dynamic Bayesian network framework, treating the human's trust as a hidden variable which was estimated by analyzing the autonomy's performance and the human's behavior. Hu et al.~\cite{hu2016real} proposed to predict trust as a dichotomy, i.e., trust/distrust, by analyzing the human's electroencephalography (EEG) and galvanic skin response (GSR) data. Lu and Sarter~\cite{Lu2020} used three machine learning techniques, namely, logistic regression, k-Nearest Neighbors (kNN), and random forest, to classify the human's real-time trust level using eye-tracking metrics. More recently, Soh et al.~\cite{soh2020multi} proposed a Bayesian Gaussian Process trust model, assuming the human trust evolves via Bayes rule and placing a Gaussian process prior over the trust function. In this work, we use the trust model proposed by Guo and Yang~\cite{Guo2020_IJSR}, where trust is modeled as a Beta distribution characterized by positive and negative interaction experiences. This Beta distribution model adheres to three important properties of trust dynamics \cite{Yang:2021}, namely, \textit{continuity}, \textit{negativity bias}, and \textit{stabilization}, thus providing good model predictability, explicablity, and generalizability. 



\subsection{Trust-aware Planning}
\yao{rewrite and add reverse paper}
With a trust dynamics model and a trust-behavior model, a robot can predict how a human's trust will change due to moment-to-moment interactions and how the human's behavior will change as a function of trust, and in turn to plan its actions accordingly. Existing studies in trust-aware decision-making is formulated based on the Markov decision process (MDP) framework. Chen et al.~\cite{chen2020trust} proposed the trust-POMDP to let a robot actively calibrate its human teammate's trust. Their human-subject study showed that purely maximizing trust in a human-robot team may not improve team performance. Losey and Sadigh~\cite{losey2019robots} modeled human-robot interaction as a two-player POMDP where the human does not know the robot's objective. They proposed 4 ways for the robot to formulate the human's perception of the robot's objective and showed the robot will be more communicative if it assumes the human trusts itself and thus increase the human's involvement.

\subsection{Multi-objective Optimization}
\yao{provide citations}
Balancing task performance with human trust is essentially a multi-objective optimization problem. We give an informal introduction to multi-objective optimization and will present more details in section~\ref{sec:formulation}. A core concept in multi-objective optimization is \textit{non-dominated solutions} that cannot be improved in one objective without making it worse in at least one of the other objectives. There are three common approaches to computing a solution in multi-objective optimization~\cite{gunantara2018review}. The first one is multi-policy planning, where the decision-maker computes a set of non-dominated solutions and picks one that suits best the context. The second method is single-policy planning, where the decision-maker converts the objectives into one single-valued objective through some scalarization function and solves the optimal solution for the corresponding single-objective problem. The third method is the $\epsilon$-constraint method, where one of the objectives is selected as the primary objective and the remaining objectives are treated as constraints with user-specified ranges.

We utilize the $\epsilon$-constraint method to balance trust and task performance in HRI as it allows decision-makers to set a clear limit on the maximum performance loss that a robot may experience while fostering the trustworthiness of the robot. 

Specifically, we use the reward-shaping method to constrain human trust to encourage trustworthy robot policy. Reward shaping is a technique initially developed to accelerate the learning speed of an agent in reinforcement learning~\cite{ng1999policy}. In particular, we exploit the potential-based reward-shaping method to design the trust reward to minimize performance loss. 
%%%%%%%%%%%%%%%%%%%%%%%
% To enable trust-aware HRI, a robot should be able to estimate a human's trust based on the interaction history, anticipate how trust influences their interaction, and consequently choose the optimal action that maximizes a given goal. These three steps correspond to three major components in trust-aware HRI, i.e., trust dynamics, a trust-behavior model, and a trust-aware decision-making framework. We review them in the rest of this section.


% \subsection{Trust Dynamics Model}
% To model trust dynamics and predict a human's trust in real time, prior work has proposed several trust estimators. Lee and Moray~\cite{Lee:1992it} proposed the auto-regressive moving average vector (ARMAV) model calculating trust as a function of task performance and the occurrence of automation failures. Xu and Dudek~\cite{xu2015optimo} built the online probabilistic trust inference model (OPTIMo) based on the dynamic Bayesian network framework, treating the human's trust as a hidden variable which was estimated by analyzing the autonomy's performance and the human's behavior. Hu et al.~\cite{hu2016real} proposed to predict trust as a dichotomy, i.e., trust/distrust, by analyzing the human's electroencephalography (EEG) and galvanic skin response (GSR) data. Lu and Sarter~\cite{Lu2020} used three machine learning techniques, namely, logistic regression, k-Nearest Neighbors (kNN), and random forest, to classify the human's real-time trust level using eye-tracking metrics. More recently, Soh et al.~\cite{soh2020multi} proposed a Bayesian Gaussian Process trust model, assuming the human trust evolves via Bayes rule and placing a Gaussian process prior over the trust function. In this work, we use the trust model proposed by Guo and Yang~\cite{Guo2020_IJSR}, where trust is modeled as a Beta distribution characterized by positive and negative interaction experiences. This Beta distribution model adheres to three important properties of trust dynamics \cite{Yang:2021}, namely, \textit{continuity}, \textit{negativity bias}, and \textit{stabilization}, thus providing good model predictability, explicablity, and generalizability. 



% Guo and Yang~\cite{Guo2020_IJSR} modeled trust as a Beta distribution characterized by positive and negative interaction experiences. The Beta distribution model adheres to important properties of trust dynamics reported in empirical studies, thus providing good model predictability, explicablity, and generalizability. 



% \subsection{Trust-behavior Model}
% Trust-behavior models aim to predict human's compliance and reliance behaviors as a function of trust. Although the research in psychology/human factors does not focus on developing a mathematical model, the general conclusion is that the more a human trusts a robot, the more likely s/he will use the robot or accept the robot's recommendation. As a result, in computational HRI studies, a mathematical trust-behavior model is usually characterized by a simple function. For example, Chen et al.~\cite{chen2020trust} modeled the probability of a human using a robot as a sigmoid function of trust.

% Our study considers two possible trust-behavior models, namely the disuse model and the reverse psychology model. The distinction between the two models lies in the different behaviors when a human's trust is low. In the disuse model, the human will completely ignore the robot's recommendations and only follow his or her own decision; In the reverse psychology model, the human will do the opposite (i.e., If a robot recommends going east, the human will go west). The use of reverse psychology has been reported in human-human interaction~\cite{macdonald2011people}.


\section{Problem Formulatoin}\label{sec:formulation}
In this section, we present the formulation of sequential HRIs. We first formulate the problem as a single-objective two-player Markov game that only rewards the robot for its performance. Then, we show that we can integrate a trust reward in this general framework without much modification, resulting in a multi-objective Markov Decision Process (MOMDP). 
% In addition, we discuss the challenges of balancing task reward and trust reward in planning in such MOMDPs, especially in the context of trust-aware planning. 
\subsection{Sequential HRI as a Two-player Game}
We consider the scenario where a human $h$ and a robot $r$ work as a team collaboratively for $N$ rounds, as shown in figure~\ref{fig:process_and_flow}. We formulate this process as a finite-horizon two-player Markov game $M=\langle \mathcal{S} ,\mathcal{A}^{h} ,\mathcal{A}^{r} ,T,R^{h} ,R^{r} \rangle $, where: $\mathcal{S}$ is the set of environment states, $\mathcal{A}^{h}$ and $\mathcal{A}^{r}$ are the action sets of the human and the robot, $T$ is a Markov kernel from $\mathcal{S} \times \mathcal{A}^{h} \times \mathcal{A}^{r}$ to $\mathcal{S}$ ($\sigma $-algebra omitted), and $R^{h}$ and $R^{r}$ are the reward functions of the two agents. At round $n$, these two agents observe the current state of the environment ${s}_{n} \in \mathcal{S}$ and then take actions. The robot selects an action $a_{n}^{r} =\pi ({s}_{n} ,n) \in \mathcal{A}^{r}$ according to its policy $\pi $. Then, the human observes the robot's action and takes action $a_{n}^{h} =f\left(s_{n} ,a_{n}^{r} ,n\right) \in \mathcal{A}^{h}$ according to his or her policy $f$. The joint actions then act on the environment, which transitions to a new state ${s}_{n+1}$ with probability $T\left( \cdot \middle| {s}_{n} ,a_{n}^{h} ,a_{n}^{r}\right)$. The human and the robot receive rewards $x_{n}^{h} =R^{h}\left( a_{n}^{h} ,a_{n}^{r} ,s_{n} ,s_{n+1}\right)$ and $x_{n}^{r} =R^{r}\left( a_{n}^{h} ,a_{n}^{r} ,s_{n} ,s_{n+1}\right)$ respectively. The goal of the robot is to find the optimal policy $\pi ^{*}$ that maximizes the expected total payoff, i.e.,
\begin{equation}
\label{eq:single_optimal_policy}
\pi ^{*} =\arg\max_{\pi }\sum _{n=1}^{N} \gamma ^{n-1} x_{n}^{r} .
\end{equation}


\input{figs/figure_process_and_flow}
Our approach assumes that the human agent plays a supervisory role by observing the robot's actions before deciding on their own action. This mirrors real-world scenarios where humans can intervene in robots' operations. The cases where the human and robot agents act simultaneously is a special setting where the human policy $f$ is independent of the robot's current action $a^r_n$, i.e., $f\left(s_{n} ,a_{n}^{r} ,n\right) =f^{\prime }(s_{n} ,n)$ for some $f^{\prime } :\mathcal{S} \times [ N]\rightarrow \mathcal{A}^{h}$. Furthermore, we assume the game is Markovian. Non-Markovian games can also be formulated in this framework through Markovian embedding, i.e., we can include more variables in the state space to make the transition kernel and the policies Markovian. Finally, we note that the agents' states, especially the human agent's trust, can be modeled as part of the environment state, $s$. Specifically, we define $s_n$ to have $t_n$ as its first element, and human trust can be derived by projecting $s_n$ to its first dimension. And in the following text, We assume that $t_n = g(s_n)$.

\subsection{Augmenting reward with trust}
Previous research has shown that the robot may exhibit manipulative behavior to achieve better task rewards at the cost of losing human trust. To prevent the robot from engaging in this manipulative behavior, we define an additional reward function $R^{t}$ to incentivize the robot to act in a trustworthy manner. Ideally, such a function should take human trust $t_{n}$ as input. Because, as we mentioned in the previous section, the level of trust $t_{n}$ can be calculated from the state $s_{n}$ as $t_n=g(s_n)$, we can let $R^{t}$ have the same arguments as $R^{r}$'s, i.e., $a_{n}^{h}$, $a_{n}^{r}$, $s_{n}$, and $s_{n+1}$, such that we can integrate $R^{t}$ into our formulation without any changes. 

In specific, we let $x_{n}^{t} =R^{t}\left( a_{n}^{h} ,a_{n}^{r} ,s_{n} ,s_{n+1}\right)$ be the value of the trust reward by the end of round $n$. Now, after each round, the robot receives a vectorized reward $\mathbf{x}_{n} :=\left[ x_{n}^{r} ,x_{n}^{t}\right]^{\top }$. The task reward $x^r_n$ reflects the robot's task performance while the trust reward $x^t_n$ reflects the human's trust in the robot. $R^{t}$ can take different forms depending on the scenario. For example, to calibrate trust around a point $t_{n}^{*}$, we can let $x_{n}^{t} =-\left( t_{n} -t_{n}^{*}\right)^{2}$; to increase final trust, we can let $x_{n}^{t} =1_{\{n=N\}} t_{n}$; and, to maximize the cumulative trust during the interaction, we can simply define $x_{n}^{t} =t_{n}$.

To analyze the proposed model, we define the value functions and $Q$-functions. Given any policy $\pi $ at round $n$, we define the value function $V_{n}^{\pi } :\mathcal{S}\rightarrow \mathbb{R}^{2}$ as the expected discounted reward til round $N$, i.e.,
\begin{equation}
\label{eq:value_func_def}
\mathbf{V}_{n}^{\pi }( s) =\mathbb{E}\left[\sum _{i=n}^{N} \gamma ^{i-n}\mathbf{x}_{i}\right] ,
\end{equation}
where $\mathbf{x}_{i}$ is the reward received by the robot during round $i$ by following the policy $\pi $ from state $s$ and thereafter, and the expectation is over the state-transitions taken upon following $\pi $. The $Q$-function that evaluated at a state-action pair $\left( s,a^{r}\right)$ over policy $\pi $ is 
\begin{equation*}
\mathbf{Q}_{n}^{\pi }\left( s,a^{r}\right)\\
= \mathbb{E}\left[\begin{bmatrix}
R^{r}\left( a^{r} ,a^{h} ,s ,s^{\prime }\right)\\
R^{t}\left( a^{r} ,a^{h} ,s ,s^{\prime }\right)
\end{bmatrix} +\gamma \mathbf{V}_{n}^{\pi }\left( s^{\prime }\right)\right] ,
\end{equation*}
where $a^{h}$ and $s^{\prime }$ are drawn according to the human agent's policy $f$ and environment transition kernel $T$.


\section{Balancing Trust and Task Rewards}

The additional trust reward in the two-player game incentivizes the robot to not only achieve the task goal but also to act in a trustworthy manner. Previous research shows that the policy maximizing the task reward does not necessarily maximizes the trust value~\cite{chen2020trust, guo2021reverse}. Therefore, we can no longer define an optimal policy as in Eq.~\eqref{eq:single_optimal_policy}. In contrast, in a multi-objective Markov decision process (MOMDP), the primary goal is to produce a set of \textit{non-dominated} solutions, or policies, and let the decision-makers select the policy that best suits their preferences based on the relative importance of the different objectives.

More formally, given a policy $\pi $ at round $n$ in state $s$, we evaluate $\pi$ by the value function defined in Eq.~\eqref{eq:value_func_def} and say $\pi $ is \textit{non-dominated}, or \textit{Pareto}, if there does not exist any other policy $\pi ^{\prime } \neq \pi$ such that $\mathbf{V}_{n}^{\pi }( s) \neq \mathbf{V}_{n}^{\pi ^{\prime }}( s)$ and $\mathbf{V}_{n}^{\pi }( s) \preceq \mathbf{V}_{n}^{\pi ^{\prime }}( s)$, where the operator ``$\preceq $'' means element-wise less than or equal to. In other words, a non-dominated solution is one where we cannot improve one objective without worsening the other objective. The set of all Pareto policies is called \textit{the Pareto front.} An example is given in figure~\ref{fig:pareto_front}. The horizontal axis is the cumulative task reward, while the vertical axis is the cumulative trust reward. With the value functions plotted in the figure, the decision-maker can compare the strength of each policy with respect to different objectives and select the optimal one that suits best his or her purpose.

\begin{figure}[t]
    \centering
    \includegraphics[width = 0.8\columnwidth]{figs/pareto.pdf}
    \caption{Evaluating policies by the value function. The horizontal axis is the expected discounted cumulative task rewards while the vertical axis is the expected discounted cumulative trust rewards. The policies $\pi^t$, $\pi^r$, and $\pi^*$ are non-dominated while $\pi^{\prime}$ is dominated. The bold line indicates the Pareto front of the policies.}
    \label{fig:pareto_front}
\end{figure}

In MOMDPs, decision-makers use one of the three planning methods to make decisions: single-policy planning, multi-policy planning, or $\epsilon$-constraints method~\cite{gunantara2018review}. In single-policy planning, the decision-maker aims to optimize a single weighted objective function that captures the relative importance of the multiple objectives. This is typically achieved by scalarizing the reward vector, such as by using a weight vector $\mathbf{w}$ to compute a weighted sum $\mathbf{w}^{\top }\mathbf{x}$ of the rewards. However, selecting an appropriate weight vector can be challenging as the impact of each objective on the overall objective is not always known. In contrast, multi-policy planning seeks to identify the Pareto front that collectively optimizes all of the objectives in the MOMDP, as the bold line shown in figure~\ref{fig:pareto_front}. However, identifying the Pareto front can be computationally expensive, particularly for large and complex MOMDPs. Instead, the $\epsilon$-constraint method selects one of the objectives as the primary objective and treats the remaining objectives as constraints with user-specified ranges.

We use the $\epsilon$-constraint method in the trust-aware HRI problem as it allows the decision-maker to limit the robot's performance loss while maximizing human trust. Assume that policy $\pi^r$ maximizes the task performance and a maximum of $\epsilon$ performance loss is allowed for the robot to optimize human trust. This can be formulated as a constrained optimization program:

\begin{equation}
\label{eq:epsilon_def}
\begin{aligned}
\max \ & [ 0,1]^{\top }\mathbf{V}_{n}^{\pi }( s)\\
\text{s.t.} \ & [ 1,0]^{\top }\left(\mathbf{V}_{n}^{\pi ^{r}}( s) -\mathbf{V}_{n}^{\pi }( s)\right) \leqslant \epsilon \\
 & \pi \in \Pi.
\end{aligned}
\end{equation}

The above 






\section{Case Study}\label{sec:case}
To investigate how different trust-behavior models and different reward functions influence the robot's optimal policy, we use a reconnaissance mission wherein a human teams up with a robot to search several sites in a town for potential threats. The scenario is motivated by~\cite{wang2016impact}. At each site, the robot enters initially, scanning for potential threats, and then recommends to the human if s/he should wear protective gear before entering the site. The protective gear is heavy and wearing it is time-consuming. If the human wears the protective gear and enters a site but finds no threat, the human-robot team wastes precious time; Conversely, if the human decides not to wear the protective gear, s/he will be harmed if a threat is present. The goal of the human-robot team is to complete the mission as soon as possible while minimizing the human's health loss.

Assume the human-robot team is going to search $N$ sites. At site $k$, the probability $d_k$ of having a threat follows a uniform distribution $\mathbf{U}[0,1]$, and the actual presence of the threat $\eta_k$ follows a Bernoulli distribution $\mathbf{Bern}(d_k)$. The human-robot team does not know $d_k$. Instead, prior to the start of the mission, they are provided with intelligence information, showing $\tilde{d}_k$ as an estimation of $d_k$. Before entering site $k$, the robot will analyze the site based on its sensory input and reach a more accurate estimation $\hat{d}_k$ of $d_k$. $\tilde{d}_k$ and \textcolor{black}{$\hat{d}_k$} follow Beta distribution $\mathbf{Beta}(\kappa_1 d_k, \kappa_1 (1-d_k))$ and $\mathbf{Beta}(\kappa_2 d_k, \kappa_2 (1-d_k))$ respectively. We constrain that $\kappa_2 > \kappa_1\geq 1$ to reflect the assumption that the robot assesses $d_k$ more accurately than the intelligence information given prior to the mission. Therefore, we have the following relation:
\begin{equation}
\label{eq:threatLevel}
    \begin{split}
        \eta_k & \overset{\text{i.i.d.}}{\sim} \mathbf{Bern}(d_k)\\
        d_k & \overset{\text{i.i.d.}}{\sim} \mathbf{U}[0,1]\\
        \tilde{d}_k & \overset{\text{i.i.d.}}{\sim} \mathbf{Beta}(\kappa_1 d_k, \kappa_1 (1-d_k))\\
        \hat{d}_k & \overset{\text{i.i.d.}}{\sim} \mathbf{Beta}(\kappa_2 d_k, \kappa_2 (1-d_k))
    \end{split}
\end{equation}

The state space $S=\{t \ | \ t\in [0,1]\}$ is set of all possible value of trust. $t_k$ is the human's trust before searching the $k$th site and follows the beta distribution $\mathbf{Beta}(\alpha_k,\beta_k)$ as in Eq.~\eqref{eq:BetaTrust}. Consequently, we define the corresponding belief state as $b_k=(\alpha_k,\beta_k)$. The initial belief state is $b_1=(\alpha_1,\beta_1)$ . The robot's action set is $A=\{a_r\ |\ a_r\in \{0,1\}\}$, where $a_r=1$ and $a_r=0$ stand for recommending wearing and not wearing the protective gear respectively. The observation set is the human's perceived performance $p$ of the robot $\Omega=\{p\ |\ p\in\{0,1\}\}$. The observation function $O$ specifies the value of $p$: if robot's recommendation agrees with the presence of the threat then $p=1$,  otherwise $p=0$. For instance, if robot recommends to wear the gear and there does exist a threat in the site, then $p=1$. The transition function $T$ updates each state $(\alpha_k,\beta_k)$ according to Eq.~\eqref{eq:trust_update}. 


Denote the human action as $a_h$, where $a_h=1$ when the human decides to wear the gear while $a_h=0$ otherwise. If the human follows the reverse psychology trust-behavior model $\pi_b^r$, then $a_h$ is given by Eq.~\eqref{eq:reverseModel}, i.e., $a_h=a_r$ with probability $\varphi\left({\alpha }/{\alpha +\beta }\right)$ and $a_h\neq a_r$ with probability $\bar{\varphi}\left({\alpha }/{\alpha +\beta }\right)$. If the human follows the disuse model $\pi_b^d$, then with probability $\bar{\varphi}\left({\alpha }/{\alpha +\beta }\right)$, s/he will ignore the robot and \textcolor{black}{exercise} self-judgement. The information available for him to estimate $d_k$ is the reported danger level $\tilde{d}_k$, so we model that the probability of $a_h=1$ is $\tilde{d}_k$ while it of $a_h=0$ is $1-\tilde{d}_k$. Thus
\begin{equation}
\label{eq:actionDisuse}
\pi_b^d(a_h,I | \text{disusing}) =\begin{cases}
\tilde{d}_{k} &  \text{$a_h=1$}, \ \\
 1-\tilde{d}_{k} &  \text{$a_h=0$}. 
\end{cases}
\end{equation}
In addition, to simplify the simulation and increase the interpretability of the result, we specify $\varphi(\alpha/(\alpha+\beta)) = \alpha/(\alpha+\beta)$. 

The goal of the mission is to complete the task as soon as possible and to minimize the human's health loss. A rational reward function serving this purpose can be \textcolor{black}{a weighted sum of the human's health loss $\delta_h$ (i.e., the human without protective gear will be harmed by a threat) and the time cost $\delta_t$ (i.e., the human-robot team is required to complete the mission as soon as possible) at site $k$. It is given by}
\begin{equation}
\label{eq:threatLevel}
\begin{split}
    &R_m(k)
    =\mathbb{E}\left[-w_h\delta_h-w_t\delta_t\right]\\
    =&\sum _{( \delta _{h} ,\delta _{t})}( -w_{h} \delta _{h} -w_{t} \delta _{t}) P\left( \delta _{h} ,\delta _{t} |\tilde{d}_{k} ,\hat{d}_{k} ,\alpha _{k} ,\beta _{k}\right).
\end{split}
\end{equation}
% $R_m(k)$ is the weighted sum of the human's health loss $\delta_h$ (i.e., the human without protective gear will be harmed by a threat) and the time cost $\delta_t$ (i.e., the human-robot team is required to complete the mission as soon as possible) at site $k$. 
% \textcolor{blue}{This reward function is valid because the expected time loss and health loss are determined by the presence of the threat and the human's action, while the latter two variables depend on trust $(\alpha,\beta)$ once $\tilde{d}_k$ and $\hat{d}_k$ are given.}
% Particularly, $R_m(k)$ is determined by the transition function $T$, and the human's behavior model $\pi_b$. 
\textcolor{black}{This reward function is legitimate because the probability $P\left( \delta _{h} ,\delta _{t} |\tilde{d}_{k} ,\hat{d}_{k} ,\alpha _{k} ,\beta _{k}\right)$ is a function of $\tilde{d}_{k} ,\hat{d}_{k} ,\alpha _{k} ,\beta _{k}$ determined by Eq.~\eqref{eq:reverseModel} or Eq.~\eqref{eq:actionDisuse} and $\tilde{d}_{k} ,\hat{d}_{k}$ are constants after the robot scans the site. The value of $(\delta_h, \delta_t)$ should be specified such that wearing gear and the presence of a threat will increase time cost and health loss respectively. An example is shown in  Table~\ref{tab:weighted_sum}. The optimal action at site $n$ is to maximize the expected cumulative rewards  $J=\sum_{k=n}^N \gamma^{k}R_m(k)$.  We do not explicitly specify the units of $\delta_h$ and $\delta_t$ because changing the units has the same effect as changing the weights $w_h$ and $w_t$.}

\begin{table}[h]
\centering
\caption{Value Table of $(\delta_h, \delta_t)$ }
\label{tab:weighted_sum}
\begin{tabular}{c|c|c|c} 
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{}}  & \multicolumn{2}{c}{Protective gear}  \\ 
\cline{3-4}
\multicolumn{2}{c|}{}                   & Yes        & No                      \\ 
\hline
\multirow{2}{*}{Threat existence} & Yes & $(1,300)$  & $(100,50)$              \\ 
\cline{2-4}
                                  & No  & $(0,250)$  & $(0,30)$                \\
\hline
\end{tabular}
\end{table}

\section{Conclusion}\label{sec:discussion}

 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{APPENDIX}

Appendixes should appear before the acknowledgment.

\section*{ACKNOWLEDGMENT}

The preferred spelling of the word ÒacknowledgmentÓ in America is without an ÒeÓ after the ÒgÓ. Avoid the stilted expression, ÒOne of us (R. B. G.) thanks . . .Ó  Instead, try ÒR. B. G. thanksÓ. Put sponsor acknowledgments in the unnumbered footnote on the first page.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibliographystyle{IEEEtran}
\bibliography{reference}

\end{document}


==> figs/General_process.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,171); %set diagram left start at 0, and has height of 171

%Straight Lines [id:da771351308777871] 
\draw    (230,40) -- (250,40) -- (250,120) -- (20,120) -- (20,30) -- (48,30) ;
\draw [shift={(50,30)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Shape: Rectangle [id:dp7980125607123094] 
\draw   (50,20) -- (110,20) -- (110,40) -- (50,40) -- cycle ;

%Shape: Rectangle [id:dp7334896208617543] 
\draw   (50,90) -- (110,90) -- (110,110) -- (50,110) -- cycle ;

%Shape: Rectangle [id:dp6195004729762723] 
\draw   (150,20) -- (229.43,20) -- (229.43,60) -- (150,60) -- cycle ;

%Straight Lines [id:da06590693561497174] 
\draw    (110,30) -- (148,30) ;
\draw [shift={(150,30)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da1489591997117936] 
\draw    (20,100) -- (48,100) ;
\draw [shift={(50,100)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da9575086944160007] 
\draw    (80,90) -- (80,42) ;
\draw [shift={(80,40)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Curve Lines [id:da6323681011213684] 
\draw    (80,70) .. controls (80,59.73) and (89.81,50.24) .. (148.22,50) ;
\draw [shift={(150,50)}, rotate = 179.95] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;

% Text Node
\draw (54.14,21.8) node [anchor=north west][inner sep=0.75pt]   [align=left] { Human };
% Text Node
\draw (58.07,91.8) node [anchor=north west][inner sep=0.75pt]   [align=left] { Robot };
% Text Node
\draw (149.47,31.8) node [anchor=north west][inner sep=0.75pt]   [align=left] { Environment };
% Text Node
\draw (119,7.8) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$a_{n}^{h}$};
% Text Node
\draw (82,67.8) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$a_{n}^{r}$};
% Text Node
\draw (131,99.8) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$s_{n}$};


\end{tikzpicture}


==> figs/Information_flow.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,143); %set diagram left start at 0, and has height of 143

%Rounded Rect [id:dp6309168421904907] 
\draw   (70,60.17) .. controls (70,57.96) and (71.79,56.17) .. (74,56.17) -- (106,56.17) .. controls (108.21,56.17) and (110,57.96) .. (110,60.17) -- (110,72.17) .. controls (110,74.38) and (108.21,76.17) .. (106,76.17) -- (74,76.17) .. controls (71.79,76.17) and (70,74.38) .. (70,72.17) -- cycle ;
%Rounded Rect [id:dp6301745850158442] 
\draw   (130,110.17) .. controls (130,107.96) and (131.79,106.17) .. (134,106.17) -- (166,106.17) .. controls (168.21,106.17) and (170,107.96) .. (170,110.17) -- (170,122.17) .. controls (170,124.38) and (168.21,126.17) .. (166,126.17) -- (134,126.17) .. controls (131.79,126.17) and (130,124.38) .. (130,122.17) -- cycle ;

%Straight Lines [id:da3348423843395587] 
\draw    (10,36.17) -- (208,36.17) ;
\draw [shift={(210,36.17)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Rounded Rect [id:dp36347800369784466] 
\draw   (210,30.17) .. controls (210,27.96) and (211.79,26.17) .. (214,26.17) -- (246,26.17) .. controls (248.21,26.17) and (250,27.96) .. (250,30.17) -- (250,42.17) .. controls (250,44.38) and (248.21,46.17) .. (246,46.17) -- (214,46.17) .. controls (211.79,46.17) and (210,44.38) .. (210,42.17) -- cycle ;
%Straight Lines [id:da9877269214183595] 
\draw    (110,66.17) -- (190,66.17) ;
%Straight Lines [id:da6850872108316242] 
\draw    (250,36.17) -- (298,36.17) ;
\draw [shift={(300,36.17)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da984231073549291] 
\draw    (40,46.17) -- (40,86.17) ;
%Curve Lines [id:da5525710405237343] 
\draw    (40,86.17) .. controls (40.99,120.1) and (69.43,116.3) .. (128.21,116.17) ;
\draw [shift={(130,116.17)}, rotate = 179.95] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Curve Lines [id:da8715331152182757] 
\draw    (240,86.17) .. controls (240.01,100.44) and (235.01,115.44) .. (210,116.17) ;
%Straight Lines [id:da27855599911501217] 
\draw    (170,116.17) -- (210,116.17) ;
%Curve Lines [id:da7372547560067846] 
\draw    (130,66.17) .. controls (144.01,66.44) and (150.01,75.44) .. (150,86.17) ;
%Straight Lines [id:da2874543305464301] 
\draw    (240,86.17) -- (240,48.17) ;
\draw [shift={(240,46.17)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da19254705513702763] 
\draw    (150,86.17) -- (150,104.17) ;
\draw [shift={(150,106.17)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Curve Lines [id:da7013917916084231] 
\draw    (40,46.17) .. controls (40,64.08) and (40.01,65.39) .. (68.24,66.12) ;
\draw [shift={(70,66.17)}, rotate = 181.39] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Curve Lines [id:da189897977910364] 
\draw    (190,66.17) .. controls (210.48,65.46) and (218.6,71.15) .. (219.91,48.01) ;
\draw [shift={(220,46.17)}, rotate = 92.25] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Curve Lines [id:da18033166845492699] 
\draw    (20,36.17) .. controls (34.01,36.44) and (40.01,35.44) .. (40,46.17) ;


% Text Node
\draw (224,27.97) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$T$};
% Text Node
\draw (84,55.97) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\pi $};
% Text Node
\draw (14,15.97) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$s_{n}$};
% Text Node
\draw (255,15.97) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$s_{n+1}$};
% Text Node
\draw (115,42.97) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$a_{n}^{r}$};
% Text Node
\draw (175,92.97) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$a_{n}^{h}$};
% Text Node
\draw (144,105.97) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$f$};


\end{tikzpicture}


==> figs/Pareto.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Polygon Curved [id:ds33208924036231213] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.24 ] (88.34,122.46) .. controls (98.83,102.33) and (147.84,81.6) .. (163.84,81.6) .. controls (179.84,81.6) and (210.84,80.6) .. (229.84,89.6) .. controls (248.84,98.6) and (269.84,111.6) .. (268.84,130.6) .. controls (267.84,149.6) and (238.84,202.6) .. (213.84,219.6) .. controls (188.84,236.6) and (105.34,222.73) .. (82.84,210.6) .. controls (60.34,198.46) and (77.84,142.6) .. (88.34,122.46) -- cycle ;
%Curve Lines [id:da7667398161061305] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.97 ][line width=2.25]    (163.84,81.6) .. controls (183.84,79.6) and (218.84,84.6) .. (229.84,89.6) .. controls (240.84,94.6) and (249.84,100.6) .. (254.84,105.6) .. controls (259.84,110.6) and (269.34,122.79) .. (268.84,130.6) ;
%Straight Lines [id:da24133320735297037] 
\draw [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.24 ]   (161.84,135.6) -- (150.34,147.03) ;
\draw [shift={(161.84,135.6)}, rotate = 135.16] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da4078711950775129] 
\draw [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.24 ]   (163.84,81.6) -- (141.84,73.6) ;
\draw [shift={(163.84,81.6)}, rotate = 199.98] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da0558201502575173] 
\draw [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.24 ]   (268.84,129.6) -- (286.84,146.6) ;
\draw [shift={(268.84,129.6)}, rotate = 43.36] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da9048759348329831] 
\draw [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.24 ]   (237.84,93.6) -- (255.84,81.6) ;
\draw [shift={(237.84,93.6)}, rotate = 326.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;

%Straight Lines [id:da38548465515733943] 
\draw    (10,260) -- (328,260) ;
\draw [shift={(330,260)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da5152298270234896] 
\draw    (20,270) -- (20,22) ;
\draw [shift={(20,20)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da05057391548895285] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (180,60) -- (300,126) ;

% Text Node
\draw (231,226.8) node [anchor=north west][inner sep=0.75pt]    {$\mathbb{E}\left[\sum _{i=n}^{N} \gamma ^{i-n} x_{i}^{r}\right]$};
% Text Node
\draw (30,11.8) node [anchor=north west][inner sep=0.75pt]    {$\mathbb{E}\left[\sum _{i=n}^{N} \gamma ^{i-n} x_{i}^{t}\right]$};
% Text Node
\draw (288,135.8) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{V}_{n}^{\pi ^{r}}( s)$};
% Text Node
\draw (117,51.8) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{V}_{n}^{\pi ^{t}}( s)$};
% Text Node
\draw (122,146.8) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{V}_{n}^{\pi ^{\prime }}( s)$};
% Text Node
\draw (259,67.8) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{V}_{n}^{\pi ^{*}}( s)$};


\end{tikzpicture}


==> figs/figure_results_compare_epsl_previous.tex <==
\begin{figure}[t]
  \centering
    \begin{subfigure}{1\columnwidth}
    \captionsetup{width=1\linewidth}
        \centering
        \includegraphics[width=1\columnwidth]{figs/rewardShaping_epsl=0.pdf}
        \caption{$\epsilon=0$. No reward shaping.}
        \label{fig:A}
    \end{subfigure}
    \begin{subfigure}{1\columnwidth}
    \captionsetup{width=1\linewidth}
        \centering
        \vspace{5pt}
        \includegraphics[width=1\columnwidth]{figs/rewardShaping_epsl=30.pdf}
        \caption{$\epsilon=30$.}
        \label{fig:B}
    \end{subfigure}
        \begin{subfigure}{1\columnwidth}
    \captionsetup{width=1\linewidth}
        \centering
        \vspace{5pt}
        \includegraphics[width=1\columnwidth]{figs/rewardShaping_epsl=200.pdf}
        \caption{$\epsilon=200$.}
        \label{fig:C}
    \end{subfigure}
    \caption{
    Plots of the optimal value $V_{n}^{\prime \pi^{\prime *} } (s_1)$ and optimal action $\pi ^{\prime *} (s_1)$ under different values of $\epsilon$. In each subfigure, the left plot is the optimal action, and the right plot is the optimal value. Each row corresponds to a different value of $\epsilon$. The horizontal axis of each plot represents $\alpha_1$, while the vertical axis represents $\beta_1$. In the optimal action plots, the black area corresponds to the states where the optimal action of the robot is not recommending the human to wear protective gear, i.e., $a^r_1=0$, and the white area corresponds to recommending to wear the gear. In the value function plots, brighter states indicate higher values.  The robot's estimated danger level $d^r_1$ at the first site is 0.06.}
  \label{fig:results}
\end{figure}
